Seed Optimization with Frozen Generator for Superior Zero-shot Low-light Enhancement

In this work, we observe that the generators, which are pre-trained on massive natural images, inherently hold the promising potential for superior low-light image enhancement against varying scenarios.Specifically, we embed a pre-trained generator to Retinex model to produce reflectance maps with enhanced detail and vividness, thereby recovering features degraded by low-light conditions.Taking one step further, we introduce a novel optimization strategy, which backpropagates the gradients to the input seeds rather than the parameters of the low-light enhancement model, thus intactly retaining the generative knowledge learned from natural images and achieving faster convergence speed. Benefiting from the pre-trained knowledge and seed-optimization strategy, the low-light enhancement model can significantly regularize the realness and fidelity of the enhanced result, thus rapidly generating high-quality images without training on any low-light dataset. Extensive experiments on various benchmarks demonstrate the superiority of the proposed method over numerous state-of-the-art methods qualitatively and quantitatively.

==> sec/3_Motivation.tex <==
\section{Motivation}
\begin{figure}[!t]
\centering
    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{pics/movitation/movitation_1110_a.pdf}
        \caption{Input image}
        \label{fig:sub1}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{pics/movitation/movitation_1110_b.pdf}
        \caption{Fine-tune random model}
        \label{fig:sub2}
    \end{subfigure}
    \vspace{0.3cm} % 在两行之间添加一些空间

    % 第二行
    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{pics/movitation/movitation_1110_c.pdf}
        \caption{Fine-tune pre-trained model}
        \label{fig:sub3}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{pics/movitation/movitation_1110_d.pdf}
        \caption{Optimize seed}
        \label{fig:sub4}
    \end{subfigure}
    \caption{Decomposition results in different settings. The seed-optimization strategy shows better performance in terms of quality.}
    \label{fig:movitation}
\end{figure}
%Recently, deep generative models have achieved impressive results on image processing tasks []-[], and many well-trained generative models using large-scale high-quality datasets have been released. These well-trained models include abundant generative knowledge involving the illumination, structure, and texture of a high-quality image, which can undoubtedly regularize the realness and fidelity of the enhanced image. This motivates us to use these deep generative priors for LIE tasks. A central question arises in the context of zero-shot learning scenarios: how can one effectively harness this pre-existing knowledge?

$\indent$ In pursuit of leveraging the generative knowledge embedded within pre-trained models for low-light image enhancement, we systematically investigated the impact of various initialization settings on Retinex decomposition. An intuitive way to leverage this generative knowledge is by taking a well-trained generator as the fundamental architecture and then fine-tuning it for image enhancement. However, such fine-tuning can disrupt the intricate generative knowledge cultivated on datasets of high-quality images. Our experiments, as illustrated in \Cref{fig:movitation} (c) and (d), reveal that although initializing with pre-trained weights enhances the decomposition quality, it falls short of mirroring the performance attainable in image generation domains.
%it does not fully capitalize on the generative model's inherent potential.

This observation led us to a novel conception: why not seek out an optimal 'seed' directly? As demonstrated in Figure \ref{fig:movitation} (b), our proposed methodology, which we refer to as the 'seed-optimization' strategy, significantly outperforms standard fine-tuning techniques in image enhancement tasks. Motivated by this, we introduce a novel Retinex-based Low-light Image Enhancement (LIE) model grounded in the double-DIP framework. Contrary to traditional backpropagation methods that adjust model parameters, our approach optimizes the input seeds, thereby preserving the integrity of the generative knowledge acquired from well-lit image scenarios. This seed-centric optimization, guided by generative knowledge, facilitates superior enhancement of low-light images without the need for any low-light dataset.

==> sec/tables/table_rebuttal_UserStudy.tex <==
\begin{table}[h]
\centering
\small
\vspace{-0.3cm}
\setlength{\abovecaptionskip}{0.1cm} % 设置标题上方的间距
\setlength{\belowcaptionskip}{0.1cm} % 设置标题下方的间距
\begin{tabular}{cccccc}
\hline
\textbf{} & \textbf{Ours} & \textbf{ZeroDCE++} & \textbf{SGZ} & \textbf{DUNP} & \textbf{NeRCo} \\ \hline
Avg.      & 3.18          & 2.67               & 2.65         & 2.59          & 2.31           \\ \hline
\end{tabular}
\caption{User Study.}
\label{rebuttal_UserStudy}
\vspace{-0.6cm}
\end{table}

==> sec/tables/table_rebuttal_abl.tex <==
\begin{table}[h]
\centering
\vspace{-0.3cm}
\setlength{\abovecaptionskip}{0.1cm} % 设置标题上方的间距
\setlength{\belowcaptionskip}{0.1cm} % 设置标题下方的间距
\begin{tabular}{cccccc}
\hline
              & \textbf{$\gamma$=0.15} & \textbf{$\gamma$=0.2} & \textbf{$\gamma$=0.25} & \textbf{w/o $G$} & \textbf{ours}  \\ \hline
\textbf{PSNR} & 10.50           & 16.51          & 15.26           & 13.70          & \textbf{18.10} \\
\textbf{SSIM} & 0.48            & 0.68           & 0.68            & 0.50           & \textbf{0.75}  \\ \hline
\end{tabular}
\caption{More ablation results.}
\label{rebuttal_ablation}
\vspace{-0.7cm}
\end{table}

==> sec/tables/table_rebuttal_appl.tex <==
\begin{table}[h]
\centering
\small
\vspace{-0.4cm}
\setlength{\abovecaptionskip}{0.1cm} % 设置标题上方的间距
\setlength{\belowcaptionskip}{0.1cm} % 设置标题下方的间距
\begin{tabular}{ccc}
\hline
              & \textbf{Top1 acc/CODaN} & \textbf{AP/Darkface} \\ \hline
baseline      & 50.16\%                 & 0.6116               \\
EnlightGAN    & 53.08\%                 & 0.6505               \\
RUAS          & 55.60\%                 & 0.6624               \\
Retinexformer & 55.07\%                 & 0.6500               \\
\textbf{Ours} & \textbf{56.40\%}        & \textbf{0.6638}      \\ \hline
\end{tabular}
\caption{Comparison of high-level application.}
\label{rebuttal_appl}
\vspace{-0.6cm}
\end{table}

==> sec/tables/table_rebuttal_computations.tex <==
\begin{table}[h]
\centering
\small
\vspace{-0.3cm}
\setlength{\abovecaptionskip}{0.1cm} % 设置标题上方的间距
\setlength{\belowcaptionskip}{0.1cm} % 设置标题下方的间距
\begin{tabular}{cccc}
\hline
        & \textbf{SIZE (M)} & \textbf{FLOPs (G)} & \textbf{TIME (S)} \\ \hline
GDP     & 552.7    & 1113.8    & 1.11     \\
DUNP    & 2.190    & 64.789    & 0.0661   \\
Ours    & 0.3640   & 11.098    & 0.00813  \\ \hline
\end{tabular}
\caption{Comparison of computing resources.}
\label{rebuttal_computation}
\vspace{-0.6cm}
\end{table}

% \begin{table}[h]
% \centering
% \small
% \vspace{-0.3cm}
% \setlength{\abovecaptionskip}{0.1cm} % 设置标题上方的间距
% \setlength{\belowcaptionskip}{0.1cm} % 设置标题下方的间距
% \begin{tabular}{cccc}
% \hline
%               & SIZE (M) & FLOPs (G) & TIME (S) \\ \hline
% ZeroDCE       & 0.0794   & 19.008    & 0.00103  \\
% RUAS          & 0.0034   & 0.78408   & 0.0196   \\
% Retinexformer & 1.606    & 62.323    & 1.74     \\
% EnlightGAN    & 8.637    & 61.026    & 0.00766  \\
% GDP           & 552.7    & 1113.8    & 1.11     \\
% DUNP          & 2.190    & 64.789    & 0.0661   \\
% Ours          & 0.3640   & 11.098    & 0.00813  \\ \hline
% \end{tabular}
% \label{rebuttal_computation}
% \caption{Compared with other state-of-the-art methods, the definitions of Rank and RoR are consistent with Table X.}
% \vspace{-0.6cm}
% \end{table}

==> sec/tables/table_rebuttal_vssota.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
% \small
\renewcommand\arraystretch{1.2}
\resizebox{2\columnwidth}{!}{%限制表格大小start
\begin{tabular}{ccccccccccccccc}
\hline
              & \multicolumn{4}{c}{\textbf{LOL}}                      & \multicolumn{2}{c}{\textbf{MEF}} & \multicolumn{2}{c}{\textbf{LIME}} & \multicolumn{2}{c}{\textbf{DICM}} & \multicolumn{2}{c}{\textbf{NPE}} & \multirow{2}{*}{\textbf{Rank}} & \multirow{2}{*}{\textbf{RoR}} \\ \cline{2-13}
              & \textbf{P↑} & \textbf{S↑} & \textbf{N↓} & \textbf{M↑} & \textbf{N↓}     & \textbf{M↑}    & \textbf{N↓}     & \textbf{M↑}     & \textbf{N↓}     & \textbf{M↑}     & \textbf{N↓}     & \textbf{M↑}    &                                &                               \\ \hline
LIME          & 14.02       & 0.62        & 8.0915      & 56.5492     & 3.4233          & 64.4771        & 3.8539          & 60.6644         & 3.7601          & 60.7453         & 4.2682          & 67.3865        & 7.6                            & 9                             \\
LLFlow-SKF    & 26.37       & 0.93        & 5.55        & 74.04       & 4.80            & 51.50          & 4.93            & 49.74           & 4.21            & 56.35           & 4.54            & 64.45          & 11.10                          & 13                            \\
Retinexformer & 25.15       & 0.90        & 3.47        & 63.15       & 3.44            & 62.16          & 3.86            & 59.45           & 3.93            & 58.32           & 3.97            & 66.22          & 7.30                           & 6                             \\
Ours          & 18.10       & 0.75        & 2.80        & 58.98       & 3.16            & 65.19          & 3.64            & 63.12           & 3.43            & 65.19           & 3.63            & 68.24          & 2.70                           & 1                             \\ \hline
\end{tabular}
}% 限制表格大小end
\label{rebuttal_vs_sota}
\caption{rebuttal vs sota}
\vspace{-0.3cm}
\end{table*}

==> sec/tables/table_rebuttal_vssota_small.tex <==
\begin{table}[h]
\centering
\small
\vspace{-0.3cm}
\setlength{\abovecaptionskip}{0.1cm} % 设置标题上方的间距
\setlength{\belowcaptionskip}{0.1cm} % 设置标题下方的间距
\begin{tabular}{ccc}
\hline
              & \textbf{Rank} & \textbf{RoR} \\ \hline
LIME          & 7.6           & 9            \\
LLFlow-SKF    & 11.10         & 13           \\
Retinexformer & 7.30          & 6            \\
\textbf{Ours} & \textbf{2.70} & \textbf{1}   \\ \hline
\end{tabular}
\caption{Compared with other state-of-the-art methods, the definitions of Rank and RoR are consistent with Table 1 in our paper.}
\label{rebuttal_vs_sota_small}
\vspace{-0.6cm}
\end{table}
